Measurement of CP violation in Bs --> J/psi phi decay

We briefly discuss measurements of CP violation in Bs --> J/psi phi decay. Both the phenomenology of Bs mixing and the importance of the measurement to searches for new physics, as well as technical details and issues with the analysis are included. While current results are consistent with the standard model, even large contributions from new physics cannot be excluded.

==> definitions.tex <==
\RequirePackage{xspace}

\newcommand{\mevcc}{\ensuremath{\mathrm{MeV}/c^2}\xspace}
\newcommand{\gevcc}{\ensuremath{\mathrm{GeV}/c^2}\xspace}

\newcommand{\invfb}{\ensuremath{\mathrm{fb^{-1}}}\xspace}
\newcommand{\invpb}{\ensuremath{\mathrm{pb^{-1}}}\xspace}

\newcommand{\ps}{\ensuremath{\mathrm{ps}}\xspace}
\newcommand{\invps}{\ensuremath{\mathrm{ps}^{-1}}\xspace}

\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}\xspace}

\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\sys}{\ensuremath{\mathrm{(sys)}}\xspace}
\newcommand{\Br}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\DG}{\ensuremath{\Delta\Gamma}\xspace}
\newcommand{\dd}{\ensuremath{\mathrm{d}}\xspace}
\newcommand{\CP}{\textit{CP}\xspace}
\newcommand{\phiS}{\ensuremath{\phi_s^{\Jpsi\Pphi}}\xspace}

\newcommand{\Bzero}{\PBz}
\newcommand{\Bs}{\PBs}
\newcommand{\Bsbar}{\PasB}
\DeclareRobustCommand{\PsBb}{\HepParticle{B}{\Pqs}{}\xspace}
\DeclareRobustCommand{\PsBH}{\HepParticle{B}{\Pqs}{H}\xspace}
\DeclareRobustCommand{\PsBL}{\HepParticle{B}{\Pqs}{L}\xspace}
\newcommand{\Bsboth}{\PsBb}
\newcommand{\BsH}{\PsBH}
\newcommand{\BsL}{\PsBL}

\newcommand{\Jpsi}{\PJgy}
\newcommand{\KSzero}{\ensuremath{\PKst}\xspace}
\DeclareRobustCommand{\Pfz}{\HepParticleResonanceFull{f}{0}{}{980}{}{}\xspace}

\newcommand{\BzeroJpsiKS}{\ensuremath{\Bzero\rightarrow\Jpsi\KSzero}\xspace}
\newcommand{\BzeroJpsiKs}{\ensuremath{\Bzero\rightarrow\Jpsi K_s}\xspace}
\newcommand{\BsJpsiphi}{\ensuremath{\Bsboth\rightarrow\Jpsi\Pgf}\xspace}
\newcommand{\BsJpsifnot}{\ensuremath{\Bsboth\rightarrow\Jpsi \Pfz}\xspace}

\newcommand{\tauLs}{\ensuremath{\tau_s^{L}}\xspace}
\newcommand{\tauHs}{\ensuremath{\tau_s^{H}}\xspace}
\newcommand{\GammaLs}{\ensuremath{\Gamma_s^{L}}\xspace}
\newcommand{\GammaHs}{\ensuremath{\Gamma_s^{H}}\xspace}


